JVNV: A Corpus of Japanese Emotional Speech with Verbal Content and Nonverbal Expressions

We present the JVNV, a Japanese emotional speech corpus with verbal content and nonverbal vocalizations whose scripts are generated by a large-scale language model. Existing emotional speech corpora lack not only proper emotional scripts but also nonverbal vocalizations (NVs) that are essential expressions in spoken language to express emotions. We propose an automatic script generation method to produce emotional scripts by providing seed words with sentiment polarity and phrases of nonverbal vocalizations to ChatGPT using prompt engineering. We select 514 scripts with balanced phoneme coverage from the generated candidate scripts with the assistance of emotion confidence scores and language fluency scores. We demonstrate the effectiveness of JVNV by showing that JVNV has better phoneme coverage and emotion recognizability than previous Japanese emotional speech corpora. We then benchmark JVNV on emotional text-to-speech synthesis using discrete codes to represent NVs. We show that there still exists a gap between the performance of synthesizing read-aloud speech and emotional speech, and adding NVs in the speech makes the task even harder, which brings new challenges for this task and makes JVNV a valuable resource for relevant works in the future. To our best knowledge, JVNV is the first speech corpus that generates scripts automatically using large language models.

==> old.tex <==
Though current LLMs can generate samples with quality as high as humans, they will still make mistakes in some cases. We observe several bad cases within the generated samples. For example, although LLMs generate the script conditioned on a given emotion, sometimes they will still produce a script with wrong or weak emotions, which we considered as Emotion Mismatching. 


Though ChatGPT can generate natural and fluent sentences, we still observe some sentences that have grammar errors or unnatural expressions. To solve this problem, we adopt perplexity to evaluate their qualities. In general, lower perplexity indicates fewer grammar errors and unnatural expressions. Therefore, after filtering out those sentences with mismatched emotions, we rank the quality of sentences with respect to their perplexity decreasingly and we select those generated sentences with lower perplexity.

Finally, we obtain natural and fluent scripts with diverse nonverbal phrases and corresponding emotions. 

\begin{table}[htb]
    \centering
    \begin{tabular}{p{0.75\linewidth}}
        \toprule
            \textbf{Prompt for generating an emotional script using a word and an NV phrase}  \\
        \midrule
            Given a word and an interjection, write a grammatically correct, reasonable, and idiomatic Japanese sentence in a/an [Emotional] tone. \\
            Make sure the sentence can effectively express [Emotion] through vivid wording and specific reasons for [Emotion]. \\
            \\
            Word: [Seed word] \\
            Interjection: [Phrase] \\
            Sentence: [Sentence] \\
            \\          
            ... ($n$ pre-defined exemplars for in-context learning) \\
            \\
            Word: [Keyword] \\
            Interjection: [Phrase] \\
            Sentence: \\
        \bottomrule
         
    \end{tabular}
    \caption{Prompt template for script generation}
    \label{tab:prompt}
\end{table}

\begin{wrapfigure}{r}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/tts.pdf}
    \caption{The proposed TTS method using mixed input representations.}
    \label{figure:phone_comb}
\end{wrapfigure}

\begin{wrapfigure}{r}{0.48\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/phone_comb.pdf}
    \caption{The number of unique arrangements of consecutive phoneme(s) of each corpus.}
    \label{figure:phone_comb}
\end{wrapfigure}

\begin{table}[htbp]
\begin{floatrow}
\capbtabbox{
    \begin{tabular}{cccc}
    \toprule
    ITA & JVNV (full set) & JVNV (core set) & JTES \\
    \midrule
    $34.64$ & $33.33$ & $33.20$ & $33.10$\\
    \bottomrule
\end{tabular}
}{
 \caption{Extended phoneme entropy of each corpus. Higher entorpy means better phonemic balance}
 \label{tab:entropy}
}
\capbtabbox{
\begin{tabular}{cccc}
        \toprule
        JVNV & JVNV-V & JTES & OGVC \\
        \midrule
        $\mathbf{94.21}$ & $87.37$ & $80.85$ & $54.69$\\
        \bottomrule
    \end{tabular}
}{
    \caption{Subjective emotion recognition accuracy ($\%$) of each corpus.}
    \label{tab:gt_recognition}
}
\end{floatrow}
\end{table}

\begin{table}[htbp]
\begin{minipage}{0.45\linewidth}
\centering
\caption{Extended phoneme entropy of each corpus. Higher entorpy means better phonemic balance}
\label{tab:entropy}
\begin{tabular}{cccc}
\toprule
ITA & JVNV (full set) & JVNV (core set) & JTES \\
\midrule
$34.64$ & $33.33$ & $33.20$ & $33.10$\\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}{0.45\linewidth}
\centering
\caption{Subjective emotion recognition accuracy ($\%$) of each corpus.}
\label{tab:gt_recognition}
\begin{tabular}{cccc}
        \toprule
        JVNV & JVNV-V & JTES & OGVC \\
        \midrule
        $\mathbf{94.21}$ & $87.37$ & $80.85$ & $54.69$\\
        \bottomrule
\end{tabular}
\end{minipage}
\end{table}

\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/phone_comb.pdf}
\caption{jghj}\label{a}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/tts.pdf}
\caption{Concrete and Constructions}
\label{a}
\end{minipage}
\end{figure}

\begin{table}
  \centering
  \setlength{\belowcaptionskip}{-.25cm}
  \setlength{\abovecaptionskip}{.1cm}
  \begin{tabular}{p{13.5cm}} 
    \toprule
    \textbf{Prompt Template for Script Generation}\\
    \midrule
    \# Task Instruction \\
    \texttt{ Given a word and an interjection, write a grammatically correct in a/an [Emotional] tone.} \\
    \texttt{ Make sure the sentence can effectively express [Emotion] through vivid wording and specific reasons for [Emotion].} \\
    \\
    \# Few-shot Exemplars  \\
    \texttt{Word: [Seed word]} \\
    \texttt{Interjection: [Phrase]} \\
    \texttt{Sentence: [Sentence]} \\
    
    \\
    \# Input and output \\
    \texttt{Word: [Seed word]} \\
    \texttt{Interjection: [Phrase]} \\
    \texttt{Sentence:} \\
    \bottomrule
  \end{tabular}
  \caption{Prompt template for script generation. Texts starting with \# are comments. We use $n=3$ demonstrations during the script generation.}
  \label{tab:prompt}
\end{table}

\begin{table}[htbp]
    \centering
    %\footnotesize
    \begin{tabular}{cccccc}
        \toprule
        Emotion & F1 & F2 & M1 & M2 & $\sum$ (hrs)\\
        \midrule
        Anger & $54$ & $76$ & $54$ & $65$ & $0.53$\\
        Disgust & $59$ & $74$ & $59$ & $66$ & $0.59$\\
        Fear & $59$ & $78$ & $59$ & $69$ & $0.65$\\
        Happiness & $58$ & $90$ & $58$ & $74$ & $0.75$\\
        Sadness & $59$ & $73$ & $59$ & $66$ & $0.82$\\
        Surprise & $67$ & $86$ & $67$ & $86$ & $0.60$\\
        \midrule
        $\sum$ (hrs) & $0.94$ & $1.11$ & $0.92$ & $0.97$ & $3.94$ \\
        \bottomrule
    \end{tabular}
    % \vspace{1cm}
    \caption{Number of utterances for each (emotion, speaker) pair in JVNV. The total duration of each speaker/emotion is shown in the last row/column.}
    \label{tab:dataset}
\end{table}


\begin{table}[t]
    \centering
    \caption{Performance of the models trained with different representations for NVs. For all models we use the same test set except for the V model, where we exclude all NVs in the test set. \textbf{Bold} indicates the best score with $p < 1e\mhyphen5$.}
    \footnotesize
    \begin{tabular}{cccccccc}
    \toprule
    Model & NV & PER-V($\downarrow$) & CER-V($\downarrow$) & MCD($\downarrow$) & F0-RMSE($\downarrow$) & MOS-Emo & MOS-JSUT \\
    \midrule
    GT       &  \ding{51}   & $13.3$ & $8.9$ &  - & - & $4.7$ & $4.3$ \\
    HiFi-GAN &  \ding{51}   & $13.5$ &$9.1$  & $3.1$ & $26.4$ & $4.1$ & $3.8$ \\
    \midrule
    V   &  \ding{55} & $12.2$ & $7.3$   &$5.9$ & $49.5$ & $2.9$ & $3.4$ \\
    \midrule
    NV+V &  code  & $10.7$ & $6.1$ & $\mathbf{6.2}$ & $\mathbf{50.9}$ & $\mathbf{2.4}$ & $\mathbf{3.5}$ \\
    Phoneme  &  phoneme & $15.6$ & $14.1$ & $6.7$ & $53.1$ & $1.9$ & $3.4$ \\
    \bottomrule
    \end{tabular}
    \label{tab:tts_result}
\end{table}

==> sections/checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{section:jvnv}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the discussion in Section~\ref{section:social_impacts}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please refer to the supplementary materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to the supplementary materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We use the same random seed for all experiments. For all results, $p$-value is computed.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to the supplementary materials.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{The sentiment polarity dict, the inappropriate word list, JNV, and JSUT are all cited.}
  \item Did you mention the license of the assets?
    \answerYes{They are all available for research. Please refer to the supplementary materials.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Please refer to Section~\ref{section:introduction} to find the url of JVNV}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{JNV and JSUT are all open-sourced and can be used for non-commercial research purposes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{JNV and JSUT are open-sourced. Their authors have obtained consent from the speakers to release their speech data. This is the same for JVNV. As for the offensive content, we removed inappropriate words from these corpora when using them. Please refer to Section~\ref{section:seed_words_with_sentiment_polarity} to find detailed information.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{Please refer to the supplementary materials.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{For the MOS test described in Section~\ref{section:tts_experiment}, we describe the potential risks to the workers using this document (Japanese): \url{http://sarulab.sakura.ne.jp/rinri_jp.pdf}.\\ For the speakers of JVNV, the potential risks are described by the company the speakers belong to. The descriptions from the author to the company, and from the company to the speakers, are all documented.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{For the recording, please refer to Section~\ref{section:jvnv}. For the subjective evaluation described in Section~\ref{section:tts_experiment}, please refer to the supplementary materials}
\end{enumerate}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/two_col.tex <==
\begin{table}[htbp]
\begin{floatrow}
\capbtabbox{
    \begin{tabular}{cccc}
    \toprule
    ITA & JVNV (full) & JVNV (core) & JTES & STUDIES \\
    \midrule
    $34.64$ & $33.33$ & $33.20$ & $33.10$ & \\
    \bottomrule
\end{tabular}
}{
 \caption{Extended phoneme entropy of each corpus. Higher entorpy means better phonemic balance.}
 \label{tab:entropy}
}
\capbtabbox{
\begin{tabular}{cccc}
        \toprule
        JVNV & JVNV-V & JTES & STUDIES & OGVC \\
        \midrule
        $\mathbf{94.21}$ & $87.37$ & $80.85$ & $62.05$ & $54.69$ \\
        \bottomrule
    \end{tabular}
}{
    \caption{Subjective emotion recognition accuracy ($\%$) of each corpus.}
    \label{tab:gt_recognition}
}
\end{floatrow}
\end{table}
